A new operation mode for depth-focused high-sensitivity ToF range finding

We introduce pulsed correlation time-of-flight (PC-ToF) sensing, a new operation mode for correlation time-of-flight range sensors that combines a sub-nanosecond laser pulse source with a rectangular demodulation at the sensor side. In contrast to previous work, our proposed measurement scheme attempts not to optimize depth accuracy over the full measurement: With PC-ToF we trade the global sensitivity of a standard C-ToF setup for measurements with strongly localized high sensitivity -- we greatly enhance the depth resolution for the acquisition of scene features around a desired depth of interest. Using real-world experiments, we show that our technique is capable of achieving depth resolutions down to 2mm using a modulation frequency as low as 10MHz and an optical power as low as 1mW. This makes PC-ToF especially viable for low-power applications.

==> related.tex <==
\section{Related work}\label{sec:related}
The working principle of time-of-flight range finding setups relies on the measurement of the time that light needs to traverse the scene, measured between emittance from the light source and acquisition at the sensor. 
The available approaches can be divided into two classes that differ in both, hardware requirements and reconstruction techniques.
% 
\paragraph{Pulsed Time-of-Flight range finding}
Pulsed ToF systems (P-ToF), such as ~\cite{Goldstein1967,Koechner1968} were the first to be employed for range finding purposes. These setups emit a single short (pico-/nanosecond) laser light pulse into the scene. The sensor then receives a delayed pulse after a certain measurement time. The time delay between emittance and acquisition is directly proportional to the distance travelled and thus the depth of the scene. There exist a number of commercial LIDAR products based on this approach. More recent pulse-based systems rely on the determination of the pulse-shape altered by scene traversal~\cite{Iddan2001,Yahav2007} and implementation of a fast image shutter in front of the sensor chip. Use cases are as diverse as 
acquiring images~\cite{Kirmani2009} or object motion~\cite{Pandharkar2011} in an ``around-the-corner'' setting , measuring 3D shape~\cite{Velten2012} or separation of light transport components~\cite{Wu2012}. 
For all these scenarios, the simplicity of the underlying concept comes at the cost of fast hardware components that are able to measure time delays in the order of picoseconds ($10^{-12}$\,s) and deliver high sensitivity to alleviate the low SNR due to short exposure times. Due to these limitations, such systems often consist of a single-pixel sensor only and, for a full 3D representation of a scene, would require time-consuming scanning of the scene. Despite these shortcomings, the strength of P-ToF systems lies in their high depth resolution. 
% 
\paragraph{Correlation time-of-flight range finding}
To overcome the need for fast and expensive electronics required for P-ToF setups, correlation ToF (C-ToF) systems have been developed. The scene is illuminated with continuous temporally modulated light, often assumed to be sinusoidal, and the sensor performs a temporal correlation measurement of the incident light with a reference (or demodulation) function, which can be understood as a coding/decoding cycle and is nowadays done in hardware~\cite{Schwarte1997,Lange2001} on a per-pixel level. The per-pixel distance to the imaged object is directly proportional to the relative phase shift between the illumination signal and the signal acquired at the sensor. As modulation and demodulation signals require to be periodic, C-ToF 
measurements inherently are limited to the unambiguity range which is inversely related to the frequency of the modulation signals.
% 
\paragraph{Depth resolution enhancements for C-ToF systems}
In comparison to P-ToF systems, correlation based ToF systems exhibit considerably lower depth resolution. This is due to the fact that C-ToF systems rely on single- or few-frequency signals such as sinusoidal or triangular~\cite{Ferriere2008} modulation and demodulation signals, which in turn renders the depth estimation more prone to errors from measurement noise~\cite{Buttgen2008}. In recent years a great amount of research has been done to mitigate effects from higher harmonics of 
such modulation-demodulation signal pairs~\cite{Payne2008,Payne2010b}. More close to our work are dual-frequency setups which try to enhance depth resolution without the loss of unambiguous measurement range by combination of a high- and low-frequency measurement~\cite{Jongenelen2010,Jongenelen2011}. More recently, Gupta et al.~\cite{Gupta2018} presented a framework for general C-ToF range finding which allows for the simulation and computation of the depth resolution performance for arbitrary modulation-demodulation signal pairs. In addition, they also use their framework to develop an optimized Hamiltonian coding function, which achieves depth resolutions up to a few mm over the full ambiguity range. 
Closely tied to the work presented in this paper, Payne et al.~\cite{Payne2011} discuss the optimal choice of duty cycle for the chosen illumination signal for the special case of sinusoidal and square illumination modulation. They point out 
that a reduction of duty cycle results in an increased peak power and thus better SNR for the illumination signal, whereat the linear relation used for phase estimation is violated.
All these approaches share the desire for improvements of the depth sensitivity over the full unambiguity range, which are inherently deemed to result in a tradeoff due to their respective relations to the modulation frequency. This is due to 
the fact, that the limited bandwidth of the illumination signal(s) directly relates to the depth variations the procedure can truthfully distinguish. 
We on the other hand propose to use a dual-measurement setup similar to~\cite{Jongenelen2010,Jongenelen2011} which, instead of trying to diminish higher harmonics, explicitly makes use of this information content: We take into account the greatly 
diminished measurement range by using pulsed illumination and a rectangular reference signal but trade it for strong increment in depth sensitivity, which is especially suited for low-power setups.
% 
